Binary Black Hole Formation with Detailed Modeling: Stable Mass Transfer Leads to Lower Merger Rates

Rapid binary population synthesis codes are often used to investigate the evolution of compact-object binaries. They typically rely on analytical fits of single-star evolutionary tracks and parameterized models for interactive phases of evolution (e.g., mass-transfer on thermal timescale, determination of dynamical instability, and common envelope) that are crucial to predict the fate of binaries. These processes can be more carefully implemented in stellar structure and evolution codes such as MESA. To assess the impact of such improvements, we compare binary black hole mergers as predicted in models with the rapid binary population synthesis code COSMIC to models ran with MESA simulations through mass transfer and common-envelope treatment. We find that results significantly differ in terms of formation paths, the orbital periods and mass ratios of merging binary black holes, and consequently merger rates. While common-envelope evolution is the dominant formation channel in COSMIC, stable mass transfer dominates in our MESA models. Depending upon the black hole donor mass, and mass-transfer and common-envelope physics, at sub-solar metallicity COSMIC overproduces the number of binary black hole mergers by factors of 2--35 with a significant fraction of them having merger times orders of magnitude shorter than the binary black holes formed when using detailed MESA models. Therefore we find that some binary black hole merger rate predictions from rapid population syntheses of isolated binaries may be overestimated by factors of ~5--500. We conclude that the interpretation of gravitational-wave observations requires the use of detailed treatment of these interactive binary phases.

==> 1Intro.tex <==



==> 3MESA_results.tex <==




==> 5Relative_Rate_Results.tex <==



==> 7Discussion.tex <==



